Computational Code-Based Privacy in Coded Federated Learning

We propose a privacy-preserving federated learning (FL) scheme that is resilient against straggling devices. An adaptive scenario is suggested where the slower devices share their data with the faster ones and do not participate in the learning process. The proposed scheme employs code-based cryptography to ensure \emph{computational} privacy of the private data, i.e., no device with bounded computational power can obtain information about the other devices' data in feasible time. For a scenario with 25 devices, the proposed scheme achieves a speed-up of 4.7 and 4 for 92 and 128 bits security, respectively, for an accuracy of 95\% on the MNIST dataset compared with conventional mini-batch FL.

==> MDPC.tex <==
% \SECTION{GOPPA CODES}\LABEL{SEC:GOPPA_CODES}
% GOPPA CODES \MARVIN{CITE THIS} ARE A CLASS OF ERROR-CORRECTION CODES THAT ARE USED MOSTLY FOR CODE BASED CRYPTOGRAPHY APPLICATIONS. FOR A GIVEN PRIME POWER $Q$ AND SOME INTEGERS $M,N,R$ SUCH THAT $RM \LEQ N \LEQ Q^M$ AND A SET OF $N$ DISTINCT ELEMENTS OF $\MATHBB{F}_{Q^M}$ CALLED $\MATHCAL{L} = \{\ALPHA_0, \ALPHA_1, \DOTS, \ALPHA_{N-1}\}$. LET $G(G) \IN \MATHBB{F}_{Q^M}[X]$ BE A POLYNOMIAL WITH $\TEXT{DEG}\{G(X)\} = R$ AND $G(\ALPHA_I) \NEQ 0, \FORALL \ALPHA_I \IN \CL$. THE GOPPA CODE IS DEFINED AS FOLLOWS
% $$\CG(\CL, G) = \LEFT\{\MATHBF{C} \MID \SUM_{I=0}^{N-1} \DFRAC{C_I}{X-\ALPHA_I} = 0  \MOD G(X), \FORALL\MATHBF{C} \IN \MATHBB{F}_Q^N\RIGHT\}$$
% GOPPA CODES ARE ALTERNANT CODES, MEANING THAT THERE ARE SUBFIELD SUBCODES OF GENERALIZED REED-SOLOMON CODES. THE GOPPA CODE $\CG(\CL,G)$ IS THEN A LINEAR CODE WITH PARAMETERS $\LEFT[N = \LVERT\CL\RVERT, K \GEQ N -MR, D\GEQ R+1\RIGHT]_Q$. FOR IRREDUCIBLE BINARY GOPPA CODES THE DISTANCE IS $D\GEQ 2R+1$. 
% \MARVIN{THIS IS JUST STH WE MIGHT NEED LATER..}

\subsection{Medium-Density Parity-Check Codes}\label{subsec:MDPC}
Medium-density parity-check (MDPC) codes are error-correcting codes that are used as a component of the McEliece cryptosystem \cite{QC-MDPC}. They are closely related to low-density parity-check (LDPC) codes, with the key difference that they are characterized by a denser parity-check matrix. %The latter were seen before as a strong candidate of being used in the McEliece cryptosystem~\cite{LDPC_MC_Eliece}, but due to their sparse parity-check matrix, low-weight codewords of the dual code can enable efficient attacks. \marvin{Citation is needed!} The last fact led researches to modifying LDPC codes into MDPC codes \cite{MDPC_proposed}, whose dual code does not have low-weight codewords. 

Since MDPC codes are mainly used in the McEliece cryptosystem, they are defined over the binary field. However, these codes can easily be extended to $q$-ary MDPC codes similar as LDPC codes are generalized. An extension to the field of real numbers is possible for MDPC codes.\temp{[CITE!]}
 
% \marvin{
%Since there exist Fountain codes implementation on coded computing where the source symbols are over the reals, we think that extension of MDPC codes to the reals. This is just for us! :-) }
\subsection{Key Generation}
Quasi-cyclic MDPC (QC-MDPC) codes are used widely in code-based cryptosystems due to their small length key sizes and plausible security level. A QC-MDPC code is generated by a parity-check matrix that is in quasi-cyclic form. The parity-check matrix needs to have medium density (weights of the rows)\cite{QC-MDPC, Tillich_MPDC}. %\temp{Under Belief-Propagation decoding,} the density of the parity-check matrix $\boldsymbol{H}_{\text{QC}}$ implies a nice trade-off, since lower density provides better error-correction capabilities (LDPC codes) while higher density sacrifices error-correction properties for better security that is crucial in cryptography. However, if a Maximum-Likelihood decoding were feasible, a denser parity-check matrix would imply better error-correction capabilities. %\marvin{Reformulate this...} 
A parity-check matrix in quasi-cyclic form implies a generator matrix $\boldsymbol{G}_{\text{QC}}$ that also enjoys quasi-cyclic properties. \AGiA{This comes too late. The main principle should be introduced earlier} In a McEliece cryptosystem, the generator matrix is the public key that is published by the owner, while the parity-check matrix is the private key that is kept secret. In the original McEliece cryptosystem, the generator matrix was modified by a scrambler and permutation matrix, that scrambled the rows and permuted the columns, in order to make it look random. However, a generator matrix of a MDPC code already is random alike, therefore the additional scrambling and permutation matrix can be omitted without any loss in the security level \cite{QC-MDPC}. 
%
%\subsection{Gradient Coding} 
%
%Gradient codes~\cite{Gradient, Gradient_extended} are a class of  erasure correcting codes that have been introduced in the context of distributed (cloud) computing to mitigate the effect of straggling servers in distributed gradient descent. \AGiA{I made several changes to the text in this section. However, we  may consider moving the first sentence to the introduction and avoiding repetion, as we will need space. Here we can just explain the concept.}   Its main principle is to split the data points into $N$ partitions, where $N$ is the number of servers, and distribute $\alpha \leq N$  partitions to each server such that  any subset of $N-\alpha+1$ servers has all $N$ data partitions. Hence, gradient codes provide resiliency against $s= \alpha -1$ straggling servers. The servers  compute  a linear combination of the local gradients\textemdash computed over the data partitions they have. The master server can then  obtain the sum of all partial gradients (over all data partitions) by decoding the received linear combinations  from the   $N - \alpha +1$ fastest servers.
%In\cite{Gradient}, an $(\alpha, N)$ gradient code \AGiA{I assume you meant $N$ here? We don't use $D$.} is defined by an encoding matrix $\bfF \in \Reals^{N\times N}$ and a decoding matrix $\bfD \in \Reals^{\binom{N}{N-s} \times N}$. The $i$-th row of $\bfF$, $i \in [N]$, specifies the linear combination of the local gradients computed by the $i$-th server, while every row of $\bfD$ corresponds to a straggling pattern and defines how the master server has to linearly combine the received gradients to obtain the summation of all partial gradients. Mathematically, this can be achieved if $$\bfD\bfF = \boldsymbol{1}_{\binom{N}{N-s}\times N }\,.$$
 
